Feasible Inference for Stochastic Volatility in Brownian Semistationary Processes

This article studies the finite sample behaviour of a number of estimators for the integrated power volatility process of a Brownian semistationary process in the non semi-martingale setting. We establish three consistent feasible estimators for the integrated volatility, two derived from parametric methods and one non-parametrically. We then use a simulation study to compare the convergence properties of the estimators to one another, and to a benchmark of an infeasible estimator. We further establish bounds for the asymptotic variance of the infeasible estimator and assess whether a central limit theorem which holds for the infeasible estimator can be translated into a feasible limit theorem for the non-parametric estimator.

==> deleted.tex <==

\chapter{Proof of coefficients for $K_1$ and $K_3$}
In chapter 4 we express the scaling constant $K_p$ in terms of the coefficients $a_2, a_3, ...$ derived from the expansion of the function $u_p(x) = |x|^p - m_p$ in terms of Hermite polynomials. We established explicit expressions for these coefficients for $K_1$ and $K_3$. Here we give the derivation of the coefficients for $K_1$. The derivation for $K_3$ is similar in structure, and only involves an additional round of integration by parts.

The Hermite polynomials are defined by 

$$H_l(x) = (-1)^l e^{\frac{x^2}{2}} \frac{d^l}{dx^l} \left( e^{-\frac{x^2}{2}} \right),$$
and form an orthogonal basis for $L^2(\mathbb{R}, w(x))$ with respect to the inner product 

$$ \langle f,g \rangle = \int_{-\infty}^{\infty} f(x) \overline{g(x)} w(x) \ \mathrm{d}x,$$
where 

$$w(x) = e^{-\frac{x^2}{2}}.$$

The Hermite polynomials are orthogonal and scaled such that 

$$ \langle H_m, H_n \rangle = \sqrt{2\pi} n! \delta_{mn},$$
thus, the coefficients of $u_1(x) = |x| - 1$ are given by 

$$ a_l = \frac{1}{\sqrt{2\pi} l!} \langle u_1, H_l \rangle.$$

Now $H_0(x) \equiv 1$, and so by the linearity of the inner product and orthogonality of the Hermite polynomials, we can ignore this term, and thus find the coefficients for $|x|$ alone. Since this is an even function, and Hermite polynomials are odd or even according to their order, we know that the coefficients $a_3, a_5, ...$ must all be zero. For even $l \geq 2$, we have 

\begin{equation*}
\begin{split}
{\sqrt{2\pi} l!}a_l &= \int_{-\infty}^{\infty} |x| H_l(x) w(x) \ \mathrm{d}x \\
&= 2 \int_{0}^{\infty} x H_l(x) w(x) \ \mathrm{d}x \\
&= 2 (-1)^l \int_{0}^{\infty} x \frac{d^l}{dx^l} \left( e^{-\frac{x^2}{2}} \right) \ \mathrm{d}x.
\end{split}
\end{equation*} 

And, after applying integration by parts, we have 


\begin{equation*}
\begin{split}
{\sqrt{2\pi} l!}a_l &= 2 (-1)^{l+1} \int_{0}^{\infty} \frac{d^{l-1}}{dx^{l-1}} \left( e^{-\frac{x^2}{2}} \right) \ \mathrm{d}x \\
&= 2 (-1)^{l+1} \left[  \frac{d^{l-2}}{dx^{l-2}} \left( e^{-\frac{x^2}{2}} \right)\right]_0^{\infty}.
\end{split}
\end{equation*} 

For $l = 2$, we have 

$$ {\sqrt{2\pi} l!}a_l = -2 \left[   e^{-\frac{x^2}{2}} \right]_0^{\infty} = 2$$
giving $a_2 = \frac{1}{\sqrt{2\pi}}$. For $l > 2$, we have 


\begin{equation*}
\begin{split}
{\sqrt{2\pi} l!}a_l &= 2 (-1)^{l+1} \left[  (-1)^{l-2} \left( e^{-\frac{x^2}{2}} \right)H_{l-2}(x) \right]_0^{\infty} \\
&= 2 H_{l-2}(0),
\end{split}
\end{equation*} 
where $H_{l-2}(0)$ is the scaled Hermite number $H_{l-2}(0) = (-1)^{\frac{l-2}{2}}(l-3)!!$, so that 

$$a_l = (-1)^{\frac{l}{2}+1} \frac{ 2(l-3)!!}{\sqrt{2\pi}l!}. $$
$ \hfill \square$
 


\chapter{`BSS' R package}
The following functions were written and compiled into a package which has been made available on Github at \url{https://github.com/phillipmurray/BSS}. The package enables simulation of $\mathcal{BSS}$ processes, model fitting using both the change of frequency method and autocorrelation function, and inference on the accumulated volatility process using the estimation techniques discussed in this thesis.


\inputencoding{utf8}
\HeaderA{bssAlphaFit}{Estimating the smoothness parameter of a Brownian semistationary process}{bssAlphaFit}
%
\begin{Description}\relax
\code{bssAlphaFit} uses the `Change of Frequency' method to estimate the smoothness parameter, \code{alpha},
of a BSS process. The COF method needs only minimal assumptions on the parametric form of the kernel,
therefore the estimate can be used in any kernel.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
bssAlphaFit(Y, p = 2)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process at any frequency.

\item[\code{p}] the power to be used in the change of frequency method. The default value is p = 2.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a single value - an estimate for the smoothness parameter alpha.
\end{Value}


\inputencoding{utf8}
\HeaderA{estimateAccumulatedVolatility}{Estimate accumulated volatility processes}{estimateAccumulatedVolatility}
%
\begin{Description}\relax
\code{estimateAccumulatedVolatility} estimates the pth power accumulated volatility process for a Brownian
semistationary process, using either parametric methods of model fitting first, or using a non-parametric
estimator for the scale factor.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
estimateAccumulatedVolatility(Y, n, p = 2, method = 'nonparametric',
  kernel = 'gamma')
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process.

\item[\code{n}] positive integer indicating the number of observations per unit of time.

\item[\code{p}] the power to evaluate the accumulated power volatility process for. Defaults to 2, in order to
estimate the accumulated squared volatility process.

\item[\code{method}] text string representing the method used to estimate the accumulated volatility. Options are \code{'acf'}, \code{'cof'}
or \code{'nonparametric'}. If \code{'acf'} is selected, model parameters are fit to the data \code{Y} using
least squares on the autocorrelation function and these parameters are used to estimate the scale factor.
If \code{'cof'} is selected, only the smoothness parameter \code{alpha} is estimated using the change of frequency
method, and then put into an asymptotic expression for the scale factor in the calculation. If \code{'nonparametric'}
is selected then the non-parametric estimator for the scale factor will be used in the calculation. Defaults to \code{'nonparametric'}.

\item[\code{kernel}] text string representing the choice of kernel when fitting the model to estimate
the scale factor parametrically. Options are \code{'gamma'} and \code{'power'}. Defaults to \code{'gamma'}.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a vector of the same length as \code{Y} which is the estimate for the
accumulated volatility process, observed from time 0 to T, at intervals of T/n. Note that the values have been
divided by m\_p in the output, so that the estimation is of the integral alone. If the non-parametric
estimator for tau\_n is used then the values will be scaled by the expectation of the squared volatility, as
per the theory.
\end{Value}




\inputencoding{utf8}
\HeaderA{gammaKernelBSS}{Simulation of gamma kernel Brownian semistationary processes}{gammaKernelBSS}
%
\begin{Description}\relax
\code{gammaKernelBSS} uses the Hybrid scheme to simulate a Brownian semistationary process from the
gamma kernel. It simulates a path where the volatility process is independent of the driving Brownian motion of the
BSS process.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
gammaKernelBSS(N, n, T, kappa = 3, alpha, lambda, sigma = rep(1, N + n
  * T + 1))
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{N}] positive integer determining the number of terms in the Riemman sum element of the
hybrid scheme calculation. Should be of order at least \code{n}.

\item[\code{n}] positive integer indicating the number of observations per unit of time. It represents the fineness or frequency of observations.

\item[\code{T}] the time interval to simulate the BSS process over.

\item[\code{kappa}] positive integer giving the number of terms to use in the 'lower' sum of the hybrid scheme. Default set to 3.

\item[\code{alpha}] the smoothness parameter of the BSS process to simulate.

\item[\code{lambda}] the exponent parameter of the BSS process to simulate.

\item[\code{sigma}] the volatility process used in the BSS simulation. This should be a vector of length \code{N + n*T + 1}
representing the sample path of sigma from -N to nT. By default this is set to by a vector of 1s so that the
Gaussian core is simulated.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a list of three objects, \code{\$core} gives the Gaussian core of the process
between 0 and T, at intervals of 1/n. \code{\$bss} gives the BSS sample path on the between 0 and T, at intervals of 1/n,
and \code{\$vol} gives the volatilty process over the same time period.
\end{Value}






\inputencoding{utf8}
\HeaderA{gammaKernelBSSFit}{Fitting gamma kernel Brownian semistationary processes}{gammaKernelBSSFit}
%
\begin{Description}\relax
\code{gammaKernelBSSFit} uses a method of moments to fit the parameters of a gamma kernel Brownian semistationary process
to a vector of observations. A least squares estimate of the parameters is obtained
by minimising the mean square error between the true gamma kernel autocorrelation function and the
empirical ACF of the data, using lags 0,...,H. The number of lags \code{num\_lags} used can be adjusted.
The volatility process does not need to be specified.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
gammaKernelBSSFit(Y, n, num_lags = 10)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process at frequency \code{n}.

\item[\code{n}] positive integer indicating the number of observations per unit of time.

\item[\code{num\_lags}] the number of lags to be used in the regression. The default is to use the first 10 lags.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a list containing the parameters \code{alpha} and \code{lambda}, and also the mean square
error \code{mse} of the least squares fit. This can be used to compare model fit when trying different kernels.
\end{Value}






\inputencoding{utf8}
\HeaderA{gammaKernelCorrelation}{Autocorrelation function for the gamma kernel}{gammaKernelCorrelation}
%
\begin{Description}\relax
\code{gammaKernelCorrelation} calculates the value of the gamma kernel autocorrelation function
directly using the analytic expression.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
gammaKernelCorrelation(alpha, lambda, h)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{alpha}] the smoothness parameter, alpha, for the gamma kernel.

\item[\code{lambda}] the exponent parameter, lambda, for the gamma kernel.

\item[\code{h}] the lag to calculate the autocorrelation at.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the autocorrelation for the gamma kernel with
parameters \code{alpha} and \code{lambda} at lag \code{h}.
\end{Value}



\inputencoding{utf8}
\HeaderA{gammaKernelTau}{Scale factor for the gamma kernel}{gammaKernelTau}
%
\begin{Description}\relax
\code{gammaKernelTau} evaluates the scale factor tau\_n for the gamma kernel using the
exact expression derived from the covariance function.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
gammaKernelTau(n, alpha, lambda)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{n}] a positive integer indicating the number of observations per unit of time.

\item[\code{alpha}] the smoothness parameter, alpha, for the gamma kernel.

\item[\code{lambda}] the exponent parameter, lambda, for the gamma kernel.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the scale factor (tau\_n) for the gamma kernel with
parameters \code{alpha} and \code{lambda}, observed at frequency \code{n} per unit of time.
\end{Value}



\inputencoding{utf8}
\HeaderA{gammaKernelTauAsymptotic}{Asymptotic scale factor for the gamma kernel}{gammaKernelTauAsymptotic}
%
\begin{Description}\relax
Asymptotic scale factor for the gamma kernel
\end{Description}
%
\begin{Usage}
\begin{verbatim}
gammaKernelTauAsymptotic(n, alpha)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{n}] a positive integer indicating the number of observations per unit of time.

\item[\code{alpha}] the smoothness parameter, alpha, for the gamma kernel.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns an approximation for the scale factor (tau\_n) for the gamma kernel with
smoothness parameter \code{alpha}, observed at frequency \code{n} per unit of time, using the asymptotic
expression for the scale factor.
\end{Value}



\inputencoding{utf8}
\HeaderA{hybridSchemeCovarianceMatrix}{Hybrid scheme covariance matrix}{hybridSchemeCovarianceMatrix}
%
\begin{Description}\relax
Generates the covariance matrix used in simulating Brownian semistationary processes by
the hybrid scheme.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
hybridSchemeCovarianceMatrix(kappa, n, alpha)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{kappa}] number of terms needed for the lower sum in the hybrid scheme.

\item[\code{n}] number of observations per unit of time, n = 1/delta.

\item[\code{alpha}] smoothness parameter used in the BSS simulation.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
Returns the covariance matrix for the lower sum in the hybrid scheme calculations.
The dimensions of the covariance matrix will be (kappa + 1) by (kappa + 1).
\end{Value}



\inputencoding{utf8}
\HeaderA{powerKernelBSS}{Simulation of power law kernel Brownian semistationary processes}{powerKernelBSS}
%
\begin{Description}\relax
\code{powerKernelBSS} uses the Hybrid scheme to simulate a Brownian semistationary process from the
power law kernel. It simulates a path where the volatility process is independent of the driving Brownian motion of the
BSS process.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
powerKernelBSS(N, n, T, kappa, alpha, beta, sigma = rep(1, N + n * T +
  1))
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{N}] positive integer determining the number of terms in the Riemman sum element of the
hybrid scheme calculation. Should be of order at least \code{n}.

\item[\code{n}] positive integer indicating the number of observations per unit of time. It represents the fineness or frequency of observations.

\item[\code{T}] the time interval to simulate the BSS process over.

\item[\code{kappa}] positive integer giving the number of terms to use in the 'lower' sum of the hybrid scheme. Default set to 3.

\item[\code{alpha}] the smoothness parameter of the BSS process to simulate.

\item[\code{beta}] the exponent parameter of the BSS process to simulate.

\item[\code{sigma}] the volatility process used in the BSS simulation. This should be a vector of length \code{N + n*T + 1}
representing the sample path of sigma from -N to nT. By default this is set to by a vector of 1s so that the
Gaussian core is simulated.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a list of three objects, \code{\$core} gives the Gaussian core of the process
between 0 and T, at intervals of 1/n. \code{\$bss} gives the BSS sample path on the between 0 and T, at intervals of 1/n,
and \code{\$vol} gives the volatilty process over the same time period.
\end{Value}



\inputencoding{utf8}
\HeaderA{powerKernelBSSFit}{Fitting power law kernel Brownian semistationary processes}{powerKernelBSSFit}
%
\begin{Description}\relax
\code{powerKernelBSSFit} uses a method of moments to fit the parameters of a power law kernel Brownian semistationary process
to a vector of observations. A least squares estimate of the parameters is obtained
by minimising the mean square error between the true power law kernel autocorrelation function (found by numerical intergration)
and the empirical ACF of the data, using lags 0,...,H. The number of lags \code{num\_lags} used can be adjusted.
The volatility process does not need to be specified.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
powerKernelBSSFit(Y, n, num_lags = 10)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process at frequency \code{n}.

\item[\code{n}] positive integer indicating the number of observations per unit of time.

\item[\code{num\_lags}] the number of lags to be used in the regression. The default is to use the first 10 lags.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns a list containing the parameters \code{alpha} and \code{beta}, and also the mean square
error \code{mse} of the least squares fit. This can be used to compare model fit when trying different kernels.
\end{Value}



\inputencoding{utf8}
\HeaderA{powerKernelCorrelation}{Autocorrelation function for the power law kernel}{powerKernelCorrelation}
%
\begin{Description}\relax
\code{powerKernelCorrelation} calculates the value of the power law kernel autocorrelation function
directly using numerical integration for the numerator (the covariance term) and the analytic expression
for the denominator (variance term).
\end{Description}
%
\begin{Usage}
\begin{verbatim}
powerKernelCorrelation(alpha, beta, h)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{alpha}] the smoothness parameter, alpha, for the power law kernel.

\item[\code{beta}] the exponent parameter, beta, for the power law kernel.

\item[\code{h}] the lag to calculate the autocorrelation at.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the autocorrelation for the power law kernel with
parameters \code{alpha} and \code{beta} at lag \code{h}.
\end{Value}


\inputencoding{utf8}
\HeaderA{powerKernelTau}{Scale factor for the power law kernel}{powerKernelTau}
%
\begin{Description}\relax
\code{powerKernelTau} evaluates the scale factor tau\_n for the power law kernel using
numerical integration for the covariance term, and exact evaluation for the variance term.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
powerKernelTau(n, alpha, beta)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{n}] a positive integer indicating the number of observations per unit of time.

\item[\code{alpha}] the smoothness parameter, alpha, for the power law kernel.

\item[\code{beta}] the exponent parameter, beta, for the power law kernel.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the scale factor (tau\_n) for the power law kernel with
parameters \code{alpha} and \code{beta}, observed at frequency \code{n} per unit of time.
\end{Value}



\inputencoding{utf8}
\HeaderA{realisedPowerVariation}{Realised power variation}{realisedPowerVariation}
%
\begin{Description}\relax
\code{realisedPowerVariation} calculates the realised power variation for a BSS process, which is then
used as a component of estimating the accumulated volatility process.
\end{Description}
%
\begin{Usage}
\begin{verbatim}
realisedPowerVariation(Y, p)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process.

\item[\code{p}] the power variation to be calculated.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the sum of the pth powers of the absolute first differences of the BSS process.
\end{Value}



\inputencoding{utf8}
\HeaderA{tauNonParametricEstimate}{Non-parametric estimate of the scale factor}{tauNonParametricEstimate}
%
\begin{Description}\relax
Non-parametric estimate of the scale factor
\end{Description}
%
\begin{Usage}
\begin{verbatim}
tauNonParametricEstimate(Y)
\end{verbatim}
\end{Usage}
%
\begin{Arguments}
\begin{ldescription}
\item[\code{Y}] a vector of observations of a BSS process.
\end{ldescription}
\end{Arguments}
%
\begin{Value}
The function returns the non-parametric estimate for the scale factor.
Note that this will be scaled by the expectation of the square of the volatility.
\end{Value}
